ASPEN: ASP-Based System for Collective Entity Resolution

In this paper, we present ASPEN, an answer set programming (ASP) implementation of a recently proposed declarative framework for collective entity resolution (ER). While an ASP encoding had been previously suggested, several practical issues had been neglected, most notably, the question of how to efficiently compute the (externally defined) similarity facts that are used in rule bodies. This leads us to propose new variants of the encodings (including Datalog approximations) and show how to employ different functionalities of ASP solvers to compute (maximal) solutions, and (approximations of) the sets of possible and certain merges. A comprehensive experimental evaluation of ASPEN on real-world datasets shows that the approach is promising, achieving high accuracy in real-life ER scenarios. Our experiments also yield useful insights into the relative merits of different types of (approximate) ER solutions, the impact of recursion, and factors influencing performance.

==> section/sim_.tex <==
% !TEX root =  ../main.tex
\def\truesim{\mathsf{Sim}_\mathsf{all}}
\def\oursim{\mathsf{Sim}_\mathsf{opt}}
\def\simfn{f_\approx}
\def\getsim{\texttt{getsim}}
\def\ubpred{\texttt{ubeq}}
Our ASP rules contain body atoms %of the form 
$\simpred_i(X,X^\prime, S)$, 
but such similarity facts are not present in the data sources 
and need to be computed via external functions. The question then is how best
to compute a sufficient set of $\simpred_i$ facts to properly evaluate the program, 
while avoiding making calls to the external functions for every possible pair of values. 

%To simplify the presentation, we will suppose there is a single
%similiarity relation $\simpred$, induced from a similarity function $\simfn$,
%but the approach generalizes to handle multiple similarity relations based upon 
%different functions. 
%needless computation  ensure that the we get the required 
%answers, while.   to ensure that we %, as naïvely comparing all constants appearing in 
%sim-comparable attributes will lead to a huge number of sim-facts.  

A naïve approach would be to compute and store
the set $\truesim(D)$, containing all facts $\simpred_i(c,d,s)$ 
such that $c$ and $d$ are data values of a form compatible with $\simpred_i$
and $s=f_i(c,d)$, with $f_i$ the function underlying the similarity relation $\simpred_i$. 
Although it requires only a polynomial number of function calls w.r.t.\ $|D|$,
it is nevertheless extremely costly on even moderately-sized databases. 
%
A first improvement would be to only consider those pairs of constants $(c,d) \in R[i] \times R'[j]$\footnote{$R[i]$ denotes the constant at position $i$ of $R$.}
such that there is a rule $\rho$ which contains an atom $\simpred_i(X,X^\prime, S)$
in which $X$ and $X'$ appear respectively in the $i$th (resp.\ $j$th) position of an $R$-atom (resp.\ $R'$-atom). However, as our experiments will show, this improved approach remains memory-consuming and its time consumption grows as the data size grows. %Another possibility would be to

Another idea would be to exploit the structure of the rules so that we 
only call the similarity functions on pairs of constants that occur in 
a similarity atom for which the rest of the rule body is satisfied. 

To this end, we may run an original program $\Pi_{(D,\Sigma)}$ but making \emph{online calls to the similarity functions}\footnote{Modern ASP solvers, e.g. \texttt{clingo}, support the syntax of external function calls~\cite{h2b-asp-2023}} by replacing literals $\simpred(X,Y,S), S\geq \delta$ with  $\texttt{sim}_\mathsf{ext}(X,Y)\geq\delta$. 
We denote by $\Pi_{(D,\Sigma_\mathsf{ext})}$ the modified program.
\textcolor{orange}{Note that online evaluation may delay the similarity computation until it is necessary, but gives only sim facts required in a single solution. If a different solution is required, sim facts will need to be recomputed.
A key observation is that the set $\{ \simpred(c,c',s) \in \bigcup\{ {M \in \ASet{\aspenc}}\} \}$ is a subset of the set of  $\simpred$ atoms in the unique stable model of $\Pi_{(D, \Sigma^\mathbf{ub})}$. 
Therefore, we consider computing the exact set of sim facts occur in $\ASet{\Pi_{(D, \Sigma^\mathbf{ub})}}$ to avoid redundant computation. For this, we could use the program $\Pi_{(D,\Sigma^{\mathsf{ub}}_\mathsf{ext})}$ while collecting all evaluated sim-facts.
Note however that this will compute only a portion of the sim-facts as those sim atoms in  rule bodies will not be evaluated if the rule heads are already derived.

We shall therefore employ a further ingredient: 

Our experiments show that this may accelerate the performances (time wise) of $\MS$ and $\PM$ see  Appendix}

For example, for rule $ \sigma_{\ex}$, we would remove %the body atom 
$\simpred(T,T^\prime, S)$ 
and instead store the compared variables ($T,T^\prime$) in a fresh relation $\getsim$ as follows:  
 \begin{align} \notag
 \getsim(T,T^\prime) \leftarrow &\aspsong(X,T,L,B), \aspsong(Y,T^\prime,L,B^\prime),  
        \\ 
        & \defneg~\emptypred(L), \linkasp(B,B^\prime). \label{modrule}
\end{align}
%(indeed it is precisely $ \linkasp$ which we aim to compute in the end!). 
Note however that the body still 
contains $ \linkasp(B,B^\prime)$, whose extension is initially unknown.
We shall therefore employ a further ingredient: an overapproximation of the $\linkasp$ facts.
For this, we could use the program $\Pi_{(D,\Sigma^{\mathsf{ub}})}$, except that we do not know how to 
evaluate similarity atoms in rule bodies. 
One option would be to weaken the bodies by dropping all similarity atoms, but this 
% similarity facts from the rules in $\Sigma^{\mathsf{ub}}$.
%However, this is 
yields a very loose approximation (cf.\ App.~\ref{app:lam}).  %\footnote{MB: do we have any results to report about this version of the approach? \changed{Leon: cora and dblp yielded nearly the cross product for ubeq, and for other datasets computing ubeq died without sim, i guess we can mention in appendix? }}. 
%Instead, we shall 
% An alternative is to run the original $\Pi_{(D,\Sigma^{\mathsf{ub}})}$ program, 
% but making \emph{online calls to the similarity functions}\footnote{Modern ASP solvers, e.g. \texttt{clingo}, support the syntax of external function calls~\cite{h2b-asp-2023}} by replacing literals $\simpred(X,Y,S), S\geq \delta$ with  $\texttt{sim}_\mathsf{ext}(X,Y)\geq\delta$. We denote by $\Pi_{(D,\Sigma^{\mathsf{ub}}_\mathsf{ext})}$ the modified program.

%\textcolor{red}{say briefly how this works, e.g. what do we need to change in the program itself or in the call to the solver so that it knows that we should compute $\simpred$ via an external call? if syntactic change to ASP program, then introduce notation for modified program where sim atoms marked as external - how about $\Sigma^{\mathsf{ub}}_\mathsf{ext}$?}%\leon{}{it is a syntatic change, where each sim literals \texttt{sim(X,Y,S), S$\geq\delta$} is replaced by $\texttt{sim}_{ext}$\texttt{(X,Y)}$\geq\delta$}. 
This will not only 
give us an 
upper bound on the true set of 
$\linkasp$ facts, but it will also compute a portion of the similarity facts
%\footnote{A further alternative would be to rely entirely on an online computation of similarity atoms over the original program. However,
%\changed{this is less efficient as results cannot be reused to compute different merge sets and may be}
%time-consuming for $\MS$ and $\PM$ solutions, c.f. App.~\ref{app:lam}. }
.
%Continuing our ongoing example, we could modify \eqref{modrule} by 
%using 

%Note that ASP solvers like 
%allow for some relations to be computed via online calls to external functions, 

%In this way, we will 
%already obtain a part of the similarity facts in this first phase, as well as the required 
%upper bound on the %true set of 
%$\linkasp$ facts.

Combining these ideas, we obtain the following %two-phase 
approach to similarity computation, on input $D, \Sigma$. % proceeds in two phases:
\begin{description}
\item[Phase 1] Compute the unique stable model $M_\mathsf{ub}$ of $\Pi_{(D,\Sigma^{\mathsf{ub}}_\mathsf{ext})}$
using %by running 
an ASP solver with external function calls enabled. 
Let $U= \{\ubpred(c,d) \mid \linkasp(c,d) \in M_\mathsf{ub}\}$,
and let $L$ contain all $\simpred_i$ facts produced during the computation. % of $M_\mathsf{ub}$. 
%upper bound + some sim facts via online calls to sim function, using $\Sigma^{\mathsf{ub}}$ program
\item[Phase 2] Let $\Pi_\simpred$ contain, for each rule $\tau$ in $\Pi_{(D, \Sigma)}$
that encodes a (soft or hard) rule in $\Sigma$ with at least one similarity atom in its body, 
a rule $\tau_\simpred$ is obtained by (i)~deleting all similarity and all comparison atoms \changed{(e.g. $ S\geq \delta$)}  from $\tau$,
(ii)~changing the head atom to $\getsim_i(T,T')$, where $\simpred_i(T,T^\prime, S)$ occurs in $\tau$,
and (iii)~renaming $\linkasp$ as $\ubpred$. 
 
\item[Phase 3] %Initialize $\oursim(D,\Sigma)$ to $L$. 
Let $M_\simpred$ be the unique stable model of $\Pi_\simpred \cup D \cup U$.
For every pair $(c,d)$ such that 
$\getsim_i(c,d) \in M_\simpred$
and there is no $\simpred_i(c,d,\_)$ fact in $L$, call 
the associated similarity function $f_i$ on input $(c,d)$,
and create the fact $\simpred_i(c,d,f_i(c,d))$. 
Let $\oursim(D,\Sigma)$ contain $L$
and all of these newly created similarity facts. %acts created by these external calls.  
\end{description}
%We %shall 
%denote by $\oursim(D,\Sigma)$ the set of similarity facts computed 
%by this approach 
%%using this approach 
%%for a %given 
%on database $D$ and %ER 
%specification $\Sigma$. 
%
Note that in Phase 2, our example rule $ \sigma_{\ex}$
would be replaced by \eqref{modrule}, but with %body atom 
$\ubpred(B,B^\prime)$ 
in place of $\linkasp(B,B^\prime)$. % replaced with $...$. 


The next %following 
result shows %us 
that this %the proposed 
approach % (\textcolor{red}{which is further detailed in the appendix})
is correct, i.e. we get the same $\linkasp$ facts using $\oursim$ 
rather than the full $\truesim$. 

%
\begin{theorem}\label{th:simCorrect}
For every database $D$ and ER specification $\Sigma$,
%\begin{align*}
\[\{M_\linkasp \mid M \in \ASet{\Pi_{(D_\mathsf{all}, \Sigma)}} \} = \{M_\linkasp \mid M \in \ASet{\Pi_{(D_\mathsf{opt}, \Sigma)}} \} \]
%$$\{M|_\linkasp \mid M \in \ASet{\Pi_{(D_\mathsf{all}, \Sigma)}} \} = \{M|_\linkasp \mid M \in \ASet{\Pi_{(D_\mathsf{opt}, \Sigma)}} \} $$
%\end{align*}
where $D_\mathsf{all}= D \cup \truesim(D)$,  $D_\mathsf{opt} = D \cup \oursim(D,\Sigma)$, 
and $M_\linkasp$ is the set of $\linkasp$\, facts in $M$. 
\end{theorem}
%NOTE: maybe want to assume that all sim atoms are guarded
%by relational atoms, since doesn't make much sense otherwise...
%\leon{}{ to also add explanation of reusing (guarding in rule bodies) eq UB to compute other solutions?} 
%%%HERE
% Note that $U$ can  be reused. Given $\Pi_\Sigma$, we obtain a variant $\Pi^\prime_\Sigma$ by appending an atom $\ubpred(X,Y)$ in the rule body for every rule in $\Pi_\Sigma$ that has a rule head $\linkasp(X,Y)$.  Let $D^\prime = D_\mathsf{opt}\cup U$, then a solution for $\Pi_{(D^\prime,\Sigma)}$ can be computed by $\Pi^\prime_{(D^\prime,\Sigma)}$.

%Note that $U$ can  be reused for solution computation. Given $\Pi_\Sigma$, we obtain a variant $\Pi^\prime_\Sigma$ by appending an atom $\ubpred(X,Y)$ in the rule body for every rule in $\Pi_\Sigma$ that has a rule head $\linkasp(X,Y)$.  Let $D^\prime = D_\mathsf{opt}\cup U$, then a solution for $D,\Sigma$ can be obtained by computing $\Pi^\prime_{(D^\prime,\Sigma)}$.  

%We now explain our approach to compute the similarity atoms in $D$  needed to evaluate the rule bodies in the ASP encoding of $(D, \Sigma)$. %Notably, the similarity assessment of a pair of constants from $D$  must be performed by calling an external function. 
%A naive approach would be to store the evaluation all possible pairs of constants that could be subject to a similarity comparison and to add the result   as atoms of the form $\simpred(X,X^\prime, S)$ to $\aspenc$.  Clearly, this approach is  computationally demanding.  To  filter out  unnecessary similarity evaluations, we use the rules in the specification  $\Sigma^{\mathsf{ub}}$. 
%A key observation is that the set $\{ \simpred(c,c',s) \in \bigcup\{ {M \in \ASet{\aspenc}}\} \}$ is a subset of the set of  $\simpred$ atoms in the unique stable model of $\Pi_{(D, \Sigma^\mathbf{ub})}$. Thus, to compute an upper bound of the required $\simpred$ atoms, we could first compute the solution of $(D, \Sigma^\mathbf{ub})$, i.e. the stable model of $\Pi_{(D, \Sigma^\mathbf{ub})}$. Note however, that such computation would still require the evaluation of \simpred atoms. To overcome this issue, we surrogate  this evaluation with a call to an external function $\olsim(X,Y)$, which computes the similarity score of $(c,c')$.  This allow us to compute an upper bound $\mathcal{E}$ of the $\linkasp$ relation, which in turn can be used to compute the $\simpred$ atoms needed as follows. 
%For each rule $r$ in $\Pi_{(D,\Sigma^\mathsf{ub})}$ and for each similarity atom $\beta = \simpred(X,X',S)$ in the body of $r$, we construct a rule  $\texttt{sim}^\prime(X,X') \leftarrow \mathbf{bd}^\prime(r)$, where $\mathbf{bd}^\prime(r)$ are all the atoms in the body of  $r$, except $\beta$. 
%The projection of the stable model of the obtained $\Pi^\mathbf{sim} \cup \mathcal{E}$ onto the $\texttt{sim}^\prime$ 
%gives us the upper bound of the required similarity atoms to find the solution for $(D, \Sigma)$. 
%






